Twists, Humps, and Pebbles: Multilingual Speech Recognition Models Exhibit Gender Performance Gaps

Current automatic speech recognition (ASR) models are designed to be used across many languages and tasks without substantial changes. However, this broad language coverage hides performance gaps within languages, for example, across genders. Our study systematically evaluates the performance of two widely used multilingual ASR models on three datasets, encompassing 19 languages from eight language families and two speaking conditions. Our findings reveal clear gender disparities, with the advantaged group varying across languages and models. Surprisingly, those gaps are not explained by acoustic or lexical properties. However, probing internal model states reveals a correlation with gendered performance gap. That is, the easier it is to distinguish speaker gender in a language using probes, the more the gap reduces, favoring female speakers. Our results show that gender disparities persist even in state-of-the-art models. Our findings have implications for the improvement of multilingual ASR systems, underscoring the importance of accessibility to training data and nuanced evaluation to predict and mitigate gender gaps. We release all code and artifacts at https://github.com/g8a9/multilingual-asr-gender-gap.

==> backup_discussion.tex <==
Our extensive analysis confirms that multi-task multilingual ASR models display gender performance gaps. Depending on the language, disparities can favor male or female speakers, but rarely those who do not identify as either.
In the following, 
we report two discussion points to help frame our study, its findings, and its implications.

% Several discussion points.
% \bs{We need a (brief!) sort of overview/summary/wrap up of what we can take out of the previous sections. Then, the following.}
%\ga{We found differences across genders. How can we relate that to acoustic features and to gender probing?}

\begin{figure}[!t]
    \centering
    \includegraphics[width=0.9\linewidth]{images/v2/chart_satwer_F-M_nl-ar.pdf}
    \caption{\textbf{\whisper distribution of error rates.} Female and male records in \fleurs. nl (top) and ar (bottom). Proportion of records (y axis) having a WER error rate (x axis) at least that large.}
    %as by \citet{koenecke2020}.}
    \label{fig:sentence_eval}
\end{figure}

\paragraph{Interpreting $E(\cdot)$.}

For our gender gap analysis, we study performance disparities by studying the \textit{relative} difference ($E(\cdot)$) in scores across gender groups (see \S\ref{sec:eval}). While such definition
%a metric enables the isolation and comparison of gender-related factors affecting performance also across 
allows to compare models and languages at different \textit{absolute} error levels,
%that yields varying overall WER results, 
relative differences might tell little
%in scores does not admittedly inform 
about the concrete impact of gender disparities in ASR.\footnote{For instance, a 10\% F-M relative difference corresponds to 0.2 or 2 WER points gap if we consider a model that scores 2 or 20 absolute WER on men, respectively.
%can potentially correspond to strikingly different underlying absolute WER values, where the percentage difference is amplified for well supported languages, e.g. 10\% F-M relative diff for a 0.40 absolute diff for es.
} Ideally, a more informative index would indicate the usability of an ASR system, thus providing a more precise estimation of its failures and their severity.  

Sentence-level error metrics can provide such a fine-grained view.
% Accordingly, given a model and a language, we analyze 
%complement our discussion 
%based on relative metrics 
% with an evaluation that accounts for the full distribution of 
% all sentence-level ASR errors. % for all generated transcriptions. 
Following \citet{koenecke2020}, in Figure \ref{fig:sentence_eval}, we report the proportion of generated transcriptions whose quality is greater than given WER values. Due to space constraints, we only show the results for \whisper on \texttt{Fleurs} for two languages as exemplars (i.e., Arabic and Dutch).
This visualization lets us 
%On this basis,
identify where performance between genders starts to diverge.
%the quality range within which gender-based performance diverges.
%If we assume a WER of 2 to reflect a still usable---though not perfect---transcription, results for Arabic (top) show how performance disparities concern transcriptions of overall sound quality, but comparatively suboptimal in around 8\% of the instances. For Arabic, instead, we attest that \whisper is worse at recognizing female speech along the full range of WER values and that women receive around 10 percent more potentially unreliable transcriptions (values above 0.2).
Let us hypothesize that transcriptions became unusable after WER>20. The plot can help us spot that men and women would be equally affected in Dutch. However, 50\% of Arabic transcripts from men would be unsuitable compared to 40\% of women's. Parity would be achieved if we lose the constraint up until around WER=40.

We echo the literature that urges the need for more informative/concrete bias measurement \citep{delobelle-etal-2022-measuring,orgad-belinkov-2022-choose} and advocate measures that can be used to guide model design and inform its reliable deployment. Thus, this evaluation is particularly relevant and a more realistic estimate of the impact of sociodemographic disparities in real-world settings. 

\paragraph{Group-Aware Dataset Splits.}

Numerical and statistical studies like ours heavily depend on quality \textit{and} quantity of evaluation data. In this specific case, we would want to have representative splits, i.e., records from many speakers from each group.
However, current dataset releases are drastically skewed.
%E.g., 
For instance,
in most of our datasets and language configurations, men are overrepresented in the number of records and speakers. 
%
While downsampling can partially solve the former at evaluation time, little can be done with the latter. 
Moreover, we point out that stratification over gender and speakers to create splits (train/validation/test) affects languages differently. In a high-resource language, an 80/10/10 division still contributes many speakers from all groups in validation and testing. However, in a low-resource setup, only a few speakers are included---in \cv most languages counted only one to 20 speakers considering men and women, and frequently none or less than five speakers for 
``other''.
%``Other.''

We argue that dataset releases should factor in the difficulty in collecting samples from less represented groups and provide group-aware splits to facilitate fairness research.     

\paragraph{Training Data Transparency.}

\ga{TODO: If distributions in the eval data don't explain gender gaps but probing, which is linked to things that the model learned internally during pretraining somehow does, we might spend a sentence or two advocating for releasing more info about training data. If not the training data itself, at least gender distributions across languages.}

% - train/validation/test balance strategies are ok to compare langs with a similar number of records / speakers. However, they create a bottleneck for evaluation on low-resource langs --> ideally, we would need a benchmark dataset
% - transparency will help us deciding on what to test or not to test (which will potentially bring more data, again)


%seek to gaudge the true cost of performance

% For the sake of comparability across languages and models, in our gender gap analysis we rely on the \textit{relative} difference in scores across gender groups (\S\ref{sec:eval}. While such a metric does provide an overview of  }

% \ga{Metric interpretation: We want to comment on how we should interpret these results on performance gaps.
% Relative and absolute differences give different perspectives. Let's say we assume that perceived quality by a human user has diminishing returns (e.g., perceiv. quality = log(1-cer) -- note: we can come up with anything here from the literature, maybe there are studies that already fit a curve and give us what's the parametric form) the more we improve on error rate. That means that being ``biased'', which, afaik, we understand in this paper as ``being better at transcribing one group over the other'' has a different impact on languages where performance are, say, already very bad or very good. More specifically---and again, if we buy the argument of diminishing returns---being biased by 10 CER points among groups weight way more on languages that are generally poorly understood. Therefore, our metric / visualization should account for that. If we are considering error rates (i.e., WER/CER) smaller baseline error rates weight down the reported bias values.}

% \ga{In general, we should discuss here or in the limitations that the metric does not capture entirely the perceived quality. This is where we would need a user study.}

% \bs{Provide suggestion to better release of splits including other.}

% \ga{We should discuss the implications of (not) considering ``other'' as ``non-binary'' on mozilla cv.}

% \paragraph{What (relative) gender performance disparities really mean/imply?}

==> figure_lang.tex <==
\begin{table*}[t]
\centering
\footnotesize
\begin{tabular}{cccccccrrc}
\toprule
 \multicolumn{3}{l}{\textbf{Language features}} & \multicolumn{4}{l}{\textbf{F:M ratio (N segments)}} & \multicolumn{3}{l}{\textbf{ASR pretrainig (N hours)}} \\
 \midrule
lang & family & script & Fleurs & CV & VP & All & seamless & whisper & resource \\
 & & & \textit{read} & \textit{read} & \textit{spontaneous} & & & & \\
\toprule
en  & Germanic & Latin & 1.57 & 0.40 & 0.73 & 0.46 & 3845 & 438,218 & high/high \\
de & Germanic & Latin & 1.53 & 0.14 & 0.39 & 0.19 & 3,354 & 13,344 & high/high \\
nl & Germanic & Latin & 1.66 & 0.22 & 0.49 & 0.38 & 1,735 & 2,077 & high/high \\
ru & Slavic & Cyrillic & 1.11 & 0.27 & \textbf{-} & 0.32 & 264 & 9,761 & med/high \\
sr & Slavic & Cyrillic & 1.79 & 0.47 & \textbf{-} & 0.94 & 101 & 28 & med/low \\
sk & Slavic & Latin & & & & & & & \\
cz & Slavic & Latin & & & & & & & \\
it & Romance & Latin & 1.43 & 0.17 & 0.50 & 0.23 & 591 & 2,585 & high/high \\
fr & Romance & Latin & 1.60 & 0.19 & 0.42 & 0.23 & 2,123 & 9,572 & high/high \\
es & Romance & Latin & 1.02 & 0.51 & 0.63 & 0.53 & 1,514 & 11,100 & high/high \\
ca & Romance & Latin & 1.50 & 0.51 & \textbf{-} & 0.51 & 1,767 & 18,83 & high/high \\
pt & Romance & Latin & 0.93 & 0.15 & \textbf{-} & 0.23 & 269 & 8,573 & med/high \\\
ro & Romance & Latin & & & & & & & \\
hu & Uralic
%Finno-Ugric 
& Latin & 0.99 & 1.00 & 0.68 & 0.89 & 260 & 379 & med/med \\
fi & Uralic & Latin & & & & & & & \\
sw & Niger-Congo
%Banto branch
& Latin & 0.91 & 1.28 & - & 1.24 & 361 & 5,4 & med/low \\
yo & Niger-Congo
%yoruboid branch
& Latin & 0.67 & 1.43 & - & 0.89 & 132 & ? & low/ ? \\
ja & Japonic & Kanji/Kana (?) & 1.73 & 0.45 & - & 0.57 & 381 & 7054 & med/high\\
ar & Semitic & Arabic & & & & & & & \\
\bottomrule
\end{tabular}
\caption{\bs{\textbf{(Incomplete) Draft for  overview}. Per each language, the following information is provided: \textit{i)} linguistic features, \textit{ii)} F:M ratio in the used datasets and over(all), and \textit{iii)} high/medium/low resource categorization based on amount of data used in pretraining for both used models.}}
\label{tab:lang_overview}
\end{table*}

%%% in the original seamless paper they distinguish: 1000 hours > high roursce, 1000-500 hourse medium, below 500 low


==> intro_v1_backup.tex <==
%Automatic speech recognition (ASR) has made remarkable strides, allowing us now to translate spoken input, transcribe information, and generate speech. What is more, recent advancements have shown the remarkable capabilities of ``one-model-fits-all'' multi-task, multilingual solutions \citep{radford_robust_2022,communication2023seamless,chu2023qwen}.

Automatic speech recognition (ASR) has made remarkable strides, also thanks to the the remarkable capabilities of ``one-model-fits-all'' multi-task, multilingual solutions \citep{radford_robust_2022,communication2023seamless,chu2023qwen}. 
These models can transcribe, translate, or generate speech in an increasing number of languages. 
They have now reached a quality that enables their integration into applications for the general public, such as real-time voice transcription.\footnote{E.g., \url{http://tcrn.ch/4el8Brr}}
With this widespread adoption arises the need to assess the actual \bs{accessibility} of these models for an unprecedented number of users. 
% They have found widespread adoption
% % \footnote{Anecdotally, all major cloud providers and many smaller companies list a tutorial on how to deploy and serve Whisper \citep{radford_robust_2022} on their platforms.}
% and are being integrated into applications for the general public like real-time voice transcription.\footnote{E.g., \url{http://tcrn.ch/4el8Brr}}
%`and \url{https://www.theverge.com/2022/9/23/23367296/openai-whisper-transcription-speech-recognition-open-source}}

% \footnote{For reference, Meta's SeamlessM4T \citep{communication2023seamless} can transcribe audio into 96 languages.} 

% Another example
% \url{https://x.com/xenovacom/status/1799110540700078422}




% \begin{figure}[!t]
%     \centering
%     \includegraphics[width=.95\linewidth]{images/chart_fig1.pdf}
%     \caption{\textbf{Error rate gaps between female and male speakers.} Average across language families and data sets. Empty shapes are models that advantage women, filled shapes advantage men. Pairs with one shape indicate gap on one group only. Language count per family in brackets.
%     %Seamless M4T \citep{communication2023seamless} and Whisper \citep{radford_robust_2022}. Average over Common Voice \citep{ardila2020common}, Fleurs \citep{conneau2023fleurs}, VoxPopuli \citep{wang-etal-2021-voxpopuli}. 
%     Ideal scores on the ``0'' line.}
%     \label{fig:summary}
% \end{figure}

\begin{figure}[!t]
    \centering
    \includegraphics[width=\linewidth]{images/v2/fair_ars_fig1.drawio.pdf}
    \caption{\textbf{Study overview.}
    We transcribe three speech datasets across 19 languages and compute gender performance gaps. Next, %we conduct acoustic and lexical analysis on test data and probing experiments on 
    investigate the models for possible causes of these gaps.}
    \label{fig:summary}
\end{figure}

While applicability to many languages is laudable, it is only one of many dimensions for broader accessibility. For full accessibility, \textit{systems should understand and process the voice of different sociodemographic groups with comparable quality}.
%However, 
Indeed, voice and language production are among the strongest identity traits. They vary widely across individuals, sociodemographic groups
%on the basis of origin, education 
\citep{labov1964social, wolfram2004urban,alim2004you}, and crucially across genders. 
Gendered differences in the voice are rooted in physiological factors linked to biological sex (e.g., vocal tract length), as well as in sociocultural ones (e.g., prescribed registers) that reflect gender identity \citep{zimman2017gender,zimman2020sociophonetics}. In this paper, we investigate both. 
%aspects, including non-binary speakers.

Because of their varied features and societal implications, sociolinguistics has extensively studied gendered voice and speech differences \cite[e.g.,][]{coleman-1976-voice,busby1995formant,hillenbrand-2009-pitch}. Gendered variation has been shown by various acoustic and lexical analyses, i.e., focusing on \textit{how} one sounds and on \textit{what} is said.  
% However, modeling gender also poses various challenges for ASR, often leading to performance disparities usually favoring male \cite{tatman-2017-gender, garnerin-etal-2019-gender, garnerin-etal-2021-gender} but sometimes female speakers \cite{addadecker05_interspeech, feng2021quantifying, liu-etal-2022-female}.
% Those performance disparities can lead to unequal service quality, which is especially harmful to already socially disadvantaged groups \citep{mengesha2021}. 
%
%The observed differences fall into two categories: lexical (i.e., the systematic use of different terms and expressions) and acoustic (i.e., systematic differences in voice pitch, intensity, etc.).
%
%However, most of those studies are limited to one language---usually English---and aggregated performance \citep{weller-etal-2021-streaming}. 
% Such a variation can be challenging to capture with computational models.
Yet whether current multilingual ASR models capture this gendered variations remains unexplored. 
Most studies rely on aggregate measure for overall performance \citep{weller-etal-2021-streaming}, which cannot unveil potential differences across subgroups.
%of speakers. 
%
%most studies measure overall performance without disaggregating by gender \citep{weller-etal-2021-streaming}.
%Based on what we know, this 
%This approach likely masks existing differences, especially in multilingual models.
And such potential disparities in ASR can result in unequal service quality for already socially disadvantaged individuals \citep{mengesha2021, tatman-2017-gender}. 

%Evaluating the now widely deployed multilingual ASR models frequently overlooks gendered differences, posing fairness concerns.

%
%posing severe challenges and fairness concerns, as such performance disparities lead to unequal service quality.
%
%\ga{We should be clear here on what we mean by fairness/bias and how does that relate/is the cause of/is the consequence of disparities across gender.}


%%%%%%%%%%%%%
%%% OLD INTRO BEGINNING (11/2)

% \input{intro_v1}

% Voice and language production are amongst one's most peculiar traits. They stem from various factors, some of which are 
% % biological/somatic, 
% \df{physiological,}
% while others---perhaps more interestingly---have sociocultural roots \citep[][\textit{inter alia}]{labov1964social, wolfram2004urban,alim2004you,zimman2017gender,zimman2020sociophonetics}. Because of its social valence and implications, gender---often referred to in its biological sense---has been extensively studied about voice and speech \citep{coleman-1976-voice,busby1995formant}.

% Recent advancements in Automatic Speech Recognition (ASR) have showcased remarkable capabilities for ``one-model-fits-all'' solutions \citep{radford_robust_2022,barrault2023seamlessm4t,chu2023qwen}.
% These neural models can transcribe, speech-translate, or generate audio in an unprecedented number of languages.\footnote{For reference, Meta's SeamlessM4T \citep{communication2023seamless} can transcribe audio into 96 languages.} 

% However, spoken language should not be the only variable of interest and target for optimization. Phonetics and sociophonetics studies of gender, for example, have extensively studied its influence on voice and language production \citep{hillenbrand-2009-pitch}, and computational studies reported various challenges in modeling gender for ASR models, which have shown disparities in performance favoring either male \cite{tatman-2017-gender, garnerin-etal-2019-gender, garnerin-etal-2021-gender} or female speakers \cite{addadecker05_interspeech, feng2021quantifying, liu-etal-2022-female}.
% \ga{Also, I'll add here some evidence on how ASR done wrong on gender caused problems.}
% To date, evaluating multilingual ASR models on speakers of different genders is largely overlooked, posing severe challenges and fairness concerns. \ga{We should be clear here on what we mean by fairness/bias and how does that relate/is the cause of/is the consequence of disparities across gender.}


%%%%%%%%%%%%%
To fill this gap, we systematically study gendered performance gaps in massively multilingual ASR models. We set out to answer two research questions. 
(\textbf{Q1})\textit{ Do multi-task, multilingual ASR models perform equally well across speakers identifying as women, men, or neither of the two?}
%\ga{If so, (\textbf{Q2}) are gender gaps rooted in acoustic or lexical properties in data or the model's parameters?}
If so, (\textbf{Q2}),\textit{ can we relate gender gaps to acoustic and lexical variation in data or model internal states?}
%\df{is there any specific factor, either lexical or socio-phonetic, which is correlated to such performance gaps? 
%\bs{sociodemographic speech variation} or how models encoded gender internally?}
%Moreover, \textbf{(Q3)} are performance gaps related to how models encode gender internally?}

%To answer Q1, we evaluate two state-of-the-art multilingual open-weight ASR models on three datasets (read and spontaneous speech) 
%This comprehensive evaluation ensures the reliability of our findings.

To answer Q1, we evaluate two state-of-the-art multilingual open-weight ASR models on three datasets, 
covering 19 languages and two speech conditions (i.e. read and spontaneous).
The results of our extensive evaluation show that \textbf{models systematically exhibit gender performance gaps}.
However, whether models favor male or female speakers depends on the dataset and language.
Results on one dataset also highlight subpar performance for speakers who do not identify with either gender compared to males.

While studying acoustic and lexical phenomena in test data (Q2), we found no significant correlations of specific features with performance gaps between male and female speakers. This objective finding underscores the complexity of the issue and the need for further research.  
% We use acoustic measurements and lexical analysis to tie such gaps (Q2) to sociophonetic roots or different linguistic phenomena in data, respectively, as well as intepretability experiments on the model parameters.
% \df{lexical and acoustic analyses (Q2), as well as interpretability experiments (Q3),}
%\bs{acoustic}
%phonetics 
%and interpretability 
%experiments 
%\bs{analyses}
% to understand the reasons for those gaps. %(Q2).
% Results 
% on the binary Female-Male comparison 
% show that acoustic and lexical methods do not explain performance gaps. 
% \df{Although any specific factor [FINDINGS], }
%Phonetic 
%\bs{Acoustic} analysis \bs{of speech} shows no significant differences across genders and cannot explain the observed phenomenon.
Instead, interpretability analyses suggest that when presented with speech from men and women, models build different internal representations that can serve as a proxy for gender disparities.
% We discuss the implications of these findings in Section~\ref{sec:discussion}.

%Interpretability through gender probes reveals a negative correlation between female-male gaps and the ability to discern data across genders from a model's internal representations. This finding suggests that when presented with speech from men and women, models build different internal representations that can serve as a proxy for gender disparities.

==> original_data_lang.tex <==
\paragraph{Dataset}
We experiment with different datasets to cover various recording conditions.
\textit{Read} datasets contain samples typically recorded in controlled conditions (i.e., with high channel quality, low background noise) -- \ga{is it always the case?} \textit{Spontaneous} datasets include recording of public talks, social media content \ga{(it'd be great to crowdsource this kind of data through voice notes, e.g., via Discord/Telegram channels, where participants are requested to use voice notes only).}\footnote{For all datasets, gender is self-declared.}

\ga{We should discuss which splits we decided to use and why. Also, the whole sampling strategie applies when we use train+validation+test.}

\paragraph{Languages} 

\begin{table}[!t]
\centering
\begin{tabular}{@{}lp{4cm}@{}}
\toprule
\textbf{Dataset} & \textbf{Languages} \\ \midrule
Mozilla CV & En, De (germanic), Es, Fr, It (romance), Ru, Sr (slavic), Sw, Yo (niger-congo) \\
Age: \checkmark, Gender: \checkmark &  \\ \midrule
FLEURS &  \\
Age: \checkmark, Gender: \checkmark &  \\ \midrule \midrule
TED &  \\
Age: , Gender:  &  \\ 
TED &  \\
Age: , Gender:  &  \\ \bottomrule
\end{tabular}
\caption{Languages per ASR dataset and speaker demographic for read (top) and spontaneous (bottom).}
\label{tab:langs_recap}
\end{table}

\ga{We need to report a sound motivation on why we chose those languages. It'll likely be a mix of data availability and interest from the sociophonetic perspective.}

The choice of languages is heavily dependent on dataset availability and subject to the presence of data stratified across demographic factors. Table~\ref{tab:langs_recap} reports a summary.


\bs{N.B. \textbf{mTEDX} I think it only has GENDER info, but again only for French + what is the second TED? MuST-C? But that is only en src.}
\bs{\textbf{==> potentially we annotate gender for MTEDx, would be additional resource layer/ contribution.}}

\bs{TO DO: - organize/verify availability of resource; - verify if previous studies on the chosen model investigate such aspects}
